A Number Representation Systems Library Supporting New Representations Based on Morris Tapered Floating-point with Hidden Exponent Bit

The introduction of posit reopened the debate about the utility of IEEE754 in specific domains. In this context, we propose a high-level language (Scala) library that aims to reduce the effort of designing and testing new number representation systems (NRSs). The library's efficiency is tested with three new NRSs derived from Morris Tapered Floating-Point by adding a hidden exponent bit. We call these NRSs MorrisHEB, MorrisBiasHEB, and MorrisUnaryHEB, respectively. We show that they offer a better dynamic range, better decimal accuracy for unary operations, more exact results for addition (37.61% in the case of MorrisUnaryHEB), and better average decimal accuracy for inexact results on binary operations than posit and IEEE754. Going through existing benchmarks in the literature, and favorable/unfavorable examples for IEEE754/posit, we show that these new NRSs produce similar (less than one decimal accuracy difference) or even better results than IEEE754 and posit. Given the entire spectrum of results, there are arguments for MorrisBiasHEB to be used as a replacement for IEEE754 in general computations. MorrisUnaryHEB has a more populated ``golden zone'' (+13.6%) and a better dynamic range (149X) than posit, making it a candidate for machine learning computations.

==> background.tex <==
This section presents the number representation systems (NRSs) and the concepts used by our library. A reader who is familiar with unary arithmetic, base 2 numbers, integer numbers, rational numbers, fractional numbers, floating-point numbers (IEEE754), tapered floating-point numbers (Morris, posit) may skip this section.

The first set of numbers introduced in computers is the natural number set $\mathbb{N}$.
There are two number representation systems for this set. The first one, called \textit{unary arithmetic} represents the value of a natural number by the number of consecutive 1s.
Unary representation is used by other NRSs. The next notations are used in this paper w.r.t. unary arithmetic: $\textit{NoC1} = \textit{Number of consecutives 1s}$, $\textit{NoC0} = \textit{Number of consecutives 0s}$, $\textit{UnaryValue} = \textit{NoC1}$.
The second system for natural numbers uses the base 2 representation of a number.
In our library, \ipnrn represents the natural NRS with infinite precision without rounding, and \fprn{n}{r} represents fixed precision with rounding, where $n$ is the size and $r$ is the type of rounding.
\ipnrn influences all the other NRSs. In the current version of our library, \ipnrn takes advantage of \texttt{Scala.BigInt}, improving performance and code readability. \fprn{n}{r} uses \ipnrn to keep the value. Most of the operations use \ipnrn operations in background and the result is converted such that it uses exactly $n$ bits. The results that need more bits are considered Not Representable (NR).

The next mathematical set is $\mathbb{Z}$, the integer numbers set. The NRS for $\mathbb{Z}$ appeared for the need to represent negative numbers. The most obvious NRS adds a bit for sign at the beginning of the representation (e.g., $0$ for positive and $1$ for negative) and the remaining bits represent the absolute value.
This system is also called \textit{sign magnitude}.
The problem with sign magnitude system is that it is representing the zero value twice as $-0$ ($10$) and $+0$ ($00$). To solve this problem, \textit{2’s complement} system uses the first bit for the sign and if the sign is negative, it gets the absolute value by negating all the bits and adding $1$.
Another system used is called \textit{bias}, where a value called bias needs to be subtracted from the binary representation to get the actual number.This system does not have a sign bit and it make possible to balance the number of positive and negative numbers that the system can represent. Usually, for $n$-bits fixed precision $\textit{bias} = 2^{n-1}-1$. Other NRSs use the bias representation with the formula $\textit{IntegerValue}=\textit{NauralBinaryValue} - bias$.
In this paper, \ipnrz represents infinite precision with no rounding sign-magnitude integer (where only $+0$ represents zero). \fprz{n}{r} represents fixed precision with rounding integer, where $n$ is the size and $r$ is the rounding.
\ipnrz uses \ipnrn to keep the absolute value and a boolean variable for the sign.
For \ipnrz, the euclidean division was chosen because of its mathematical proprieties. The power operation will inverse the number and then will apply power to the absolute value if the power is negative. The $n$-order root returns NR if the number is negative and the order is even. Similar to division, $n$-order root keeps the remainder positive by increasing the absolute value of the result by one, if necessary. \fprz{n}{r} is similar to \fprn{n}{r}. It uses \ipnrz as the value keeper. If the value is using more bits than the given size, the number becomes NR.

Next, there is $\mathbb{Q}$, the rational number set. The simplest way to represent rational numbers is to use a fractional system where the numerator is an integer number and the denominator is a natural number. The problem with the fractional system is that it can overflow easy and there are multiple ways to represent the same value. The advantage of the fractional system is that it can represent the entire rational number set $\mathbb{Q}$ in infinite precision. The overflow problem has a partial solution in doing the greater common divisor of the numerator and denominator and dividing both by its value. This solution does not solve the entire problem and adds considerable computation time. 
%%% TODO - Redundant
% Because of the increased computation time and the perfect accuracy fractional system can be used to compute the correct answer of a computation but cannot be a viable solution in an application system where time is a requirement. 
\ipnrq represents the infinite precision with no rounding fractional system. \fprq{n}{m}{r} is used for fixed precision with rounding fractional system where $n$ is the size of the numerator, $m$ is the size of the denominator, and $r$ is the type of rounding used. An extension of \fprq{n}{m}{r} proposed to solve the overflow problem is to divide by two (shifting right by one) both the numerator and denominator when one of them is out of the given size. The power function treats the negative power the same as \ipnrz. When the power is of the form $\frac{1}{x}$, the $n$-order root of the numerator and denominator are computed. If the form is $\frac{x}{1}$ then both are raised to the power of $x$. When the power has the form of $\frac{x}{y}$ with $x \neq 1$ and $y \neq 1$, then the operation of raising to $x$ is done first, and then the result is raised to the power of $\frac{1}{y}$. The size-constrained \fprq{n}{m}{r} uses \ipnrq to keep its value.

A hardware-friendly and efficient NRS for the rational number set is the \textit{fixed point} representation. It is similar to \textit{2’s complement} integer NRS, but it has an attribute called \textit{binary point}. In a simple way, the value given by the 2’s complement integer NRS is divided by two to the power of the value of the binary point. This system has an overflow problem. Its range of values is smaller than an integer NRS. \ipnrfixedp represents infinite precision with no rounding fixed point system. \fprfixedp{is}{fs}{r} is used for fixed precision with rounding fixed point system, where $is$ represents the integer size, $fs$ is the binary point value (fraction size), and $r$ is the type of rounding used. 
\ipnrfixedp keeps its value as an \ipnrq. The only requirement for this NRS is that the denominator needs to be a power of two. \fprfixedp{is}{fs}{r} takes another approach by keeping its value as a \ipnrz. The power function is done by separating the power into two parts: the integer and the fractional parts. The integer power is used for accumulating square powers ($x, x^2, x^4, ...$), while the fractional power is used for accumulating square roots ($x, \sqrt{x}, \sqrt{\sqrt{x}}, ...$).

To solve the problem of small range of values, floating-point system was proposed. In the floating-point system, the number is represented as $(-1)^{sign} \times 2^{exponent}  \times 1.f$. In infinite precision $1.f$ can be seen as a \ipnrfixedp with values inside the $[1,2)$ interval. The first bit represents the sign of the number, the next $es$ (exponent size) bits represent the exponent (usually as a bias integer NRS) and the remaining $fs$ (fraction size) bits represent the fraction bits (usually, there is a hidden bit with the value $1$ which is the most significant bit). The value is given by $(-1)^{sign} \times 2^{exponent}  \times (1+\frac{f}{2^{fs}})$, where $f=\textit{fraction bits value without hidden bit}$. A problem with the floating-point system is that $0$ cannot be represented. A solution is that when all bits except the sign bit are $0s$, the number is $0$. This creates the problem of having $+0$ and $-0$. In this paper, \ipnrfloatp represents infinite precision with no rounding floating-point NRS.
%%% TODO - not connected
%Having $+0$ and $-0$, the adding of $+\infty$ and $-\infty$ were next. 
Given its infinite precision, \ipnrfloatp does not have the concept of $\infty$. We use \floatp{fs} to represent a floating-point system with infinite precision exponent, no rounding, and with $fs+1$ (fraction size) bits of mantissa. It always has the hidden bit with the value of $1$, so the mantissa is in $[1,2)$. It also incorporates the concept of $+\infty$ and $-\infty$. Additionally, it contains a vector of extra bits used for rounding. The next NRSs are derived from it, with different rules for the range of the exponent, underflow, overflow, rounding, and binary representation. One of these NRSs is \fprfloatp{es}{fs}{r}, used for finite precision with rounding, where $es$ is the exponent size, $fs$ is the fraction size, and $r$ is the type of rounding. \fprfloatp{es}{fs}{r} rules are: (i) in the case of underflow, the value is round to zero when the exponent is smaller than the minimum exponent and the rounding rule does not change this; (ii) in the case of overflow, the value goes to $\infty$ if the exponent value is greater than the maximum exponent; (iii) the exponent is in bias form. To represent $\infty$, all the bits except the sign bit are $1$.

The second floating-point system is the standard called IEEE754~\cite{zuras2008ieee}. This NRS introduced special cases for the smallest and biggest exponent values. When the exponent has the minimum value, the hidden bit is zero and the numbers are called subnormals, except for $+0$ and $-0$. The value of subnormals is given by $(-1)^{sign} \times 2^{\text{-bias}+1} \times (0+\frac{f}{2^{fs}})$, and the process is called gradual underflow. For maximum exponent value, different bit strings for fraction and sign bit can represent \textit{qNaN} (quiet Not A Number - NaN - where the first bit of the fraction is 1), \textit{sNaN} (signal NaN, where the first bit of the fraction is 0, but there is another bit in the fraction different from 0), $+\infty$ (all fraction bits are 0), and $-\infty$ (the same as $+\infty$ only that the sign is negative). \fprieee{es}{fs}{r} represents the finite precision with rounding IEEE754 system, where $es$ is the exponent size, $fs$ is the fraction size, and $r$ is the type of rounding, and the other rules are similar to \fprfloatp{es}{fs}{r}.
\ipnrfloatp keeps its exponent value in a \ipnrz and mantissa in a \ipnrfixedp.

In our library, \floatp{fs} does not have a binary representation, but it is used for implementing other NRSs. It is a super-class NRS. It has a boolean value for the sign, an \ipnrz exponent, a \ipnrn mantissa, some bits used for rounding and the fraction size value. It implements all the operations with the scope of having a mantissa in the range $[1,2)$ by making sure that every operation produces at least $fs + 1$ bits of mantissa with the most significant one having the value $1$, except for the case when the result is $+0$ or $-0$ and the mantissa is $0$. All the additional bits produced by the operation are appended to the rest bits list. The power function is similar to \fprfixedp{is}{fs}{r} by separating the integer and fractional parts of the power. This super-class is used further by \fprfloatp{es}{fs}{r} and \fprieee{es}{fs}{r}. \fprfloatp{es}{fs}{r} and \fprieee{es}{fs}{r} are doing the operations using \floatp{fs} and then verifying the results with their rules for underflow, overflow, and binary representation. Specifically, in the case of \fprieee{es}{fs}{r}, if the exponent is smaller or equal to the minimum exponent value the number might be a subnormal number. This is tested by the difference between the subnormal exponent and the exponent value. If it is not a subnormal number, it underflows to $0$.

Beside issues such as multiple representations for zero, subnormal numbers, and too many bit representations for NaN, IEEE754 might have an oversized or undersized exponent for a given problem. Morris observed this and introduced tapered floating-point \cite{morris1971tapered}, adding an extra field representing the exponent size. This means that the exponent size and the fraction size are dynamically computed. A Morris floating-point system is determined by the total size and the size of the exponent denoted by $g$. The first $g$ bits represent the $G$ value which is used to compute the exponent size as $es = G + 1$. The next bit is the exponent sign bit followed by $es$ bits that represent the absolute value of the exponent. The next bit is the fraction sign, and the remaining bits are considered the fraction bits. The hidden bit is always $1$. The final value is computed as $2^{\text{exponent}} \times (-1)^{\textit{fraction sign}} \times (1+\frac{f}{2^{fs}})$, where  $\textit{exponent}=(-1)^{\textit{exponent sign}} \times \textit{exponentBinaryValue}$ (\textit{exponentBinaryValue} is a natural number, not in bias form). Zero is represented by all bits of zero value and error cases (NaN) are represented when all the bits are one. Small numbers have a better precision because more fraction bits are allocated to represent them. In most cases, the dynamic range of Morris NRSs is bigger compared to IEEE754 of the same size, for the obvious reason that more bits can be used for the exponent. These two proprieties give the name \textit{tapered floating-point} to Morris NRSs. On the other hand, these NRSs still have the issue of multiple representations for the same value. In this paper, we use \fprmorris{n}{g}{r} to represent finite precision with rounding Morris tapered floating-point NRS, where $n$ is the total size, $g$ is the size of the exponent, and $r$ is the type of rounding. Similar to \floatp{fs}, \taperedfloat{n} was created to help with implementing all the operations for tapered floating-point NRSs. In this case, the fraction size is not known so the system uses the total size as the exact fraction size. The fraction has a hidden bit with value $1$ and it is in the range $[1,2)$. This NRS does not represent $\infty$. Every NRS derived from it needs to add rules for underflow, overflow, rounding, and binary representation.

In trying to solve the problems of current floating-point systems, Gustafson proposed posit~\cite{gustafson2017beating} (which is another type of \taperedfloat{n}). A posit NRS is determined by its size and exponent size ($es$). The first bit in a posit s-layer representation is the sign bit. The concept for negative numbers is similar with 2's complement: all the bits are negated, and one is added to the value. Next, is the regime field which is dynamic and uses unary arithmetic representation. If the regime starts with a bit $1$, then it is a positive regime and the consecutive $1s$ are counted until a $0$ is found or the end of the representation is reached. The value of the regime is $\text{NoC1} - 1$. Otherwise, if the regime starts with a $0$, then it is a negative regime and the consecutive $0s$ are counted until the first bit of $1$ is found or the end of the representation is reached. The regime value in this case is $-1 \times \text{NoC0}$. After the regime bits, the next exponent size ($es$) bits represent the exponent value in a base 2 natural number NRS, and the remaining bits are considered fraction bits. The hidden bit is always $1$. The final value of a posit is given by $(-1)^{\textit{sign}} \times 2^{\textit{regime} \times 2^{es} + \textit{exponentBinaryValue}} \times (1+\frac{f}{2^{fs}})$. There are two special cases: for zero, all the bits are $0$, and for $NaR$ (Not a Real - positive infinity and negative infinity), first bit is $1$ and the others are $0$.

Posit solves the problem of a value having multiple representations. This is a strong propriety for an NRS. Like Morris tapered floating-point system, posit has better precision for small number creating a posit ``golden zone'' where all the operations have a better accuracy than other NRSs. In this paper, \fprposit{n}{es}{r} is used to represent fixed precision with rounding posit NRS, where $n$ is the size of the number, $es$ is the exponent size, and $r$ is the type of rounding. \fprposit{n}{es}{r} underflows to the minimum value that is not $0$ and overflows to the maximum value but not $\infty$. \fprmorris{n}{g}{r} underflows to $0$ and overflows to NR. \fprposit{n}{es}{r} is firstly creating the binary representation for the absolute value and then, if the sign is negative it subtracts one and negates all the bits. The regime bits follow the sign bit and then, depending on the remaining bits, we have the exponent bits followed by the fraction bits without the hidden bit. \fprmorris{n}{g}{r} binary representation starts with the sign. The next $g$ bits represent the minimum size for the exponent absolute value, followed by the exponent sign bit, the exponent bits, and the fraction bits without the hidden bit.


==> implementation.tex <==

This section presents the flow and decisions taken through the implementation of the library. First of them is \ipnrn. On the alpha version of the library a list of booleans was used to keep the value in base 2. \ipnrn influence all the other NRSs. This choice in implementing made the library to have a weak performance in computation time. In the current version of the library \ipnrn take advantage of Scala.BigInt, improving performance and code readability. \fprn{n}{r} use \ipnrn to keep its value. Most of the operations use \ipnrn operations in background and the result is converted to take exactly n bits given by the size. The results that needs more bits are considered NR (Not Representable). Division on \fprn{n}{r}is shifting left by two the value of the dividend, so when the division is made on \ipnrn the last 2 bits of the representation are g and r bits. The last rounding bit s is given by the remainder of the division. The result is shift right by 2 and with the values of l,g,r and s the rounding is done. The same process goes for the n order root. The number is shifted left by $2 \times n$, so the g and r bits can be computed.
\ipnrz use \ipnrn to keep the absolute value and a boolean variable for the sign. The integer division is a debated issue. There are truncated division, floored division, euclidean division, rounded division, ceiling division. For \ipnrz the euclidean division was chosen, because of its mathematical proprieties. In euclidean division the next formula: $Dividend = Divisor \times Quotient + Remainder$ with the property that the $Remainder \geq 0$ holds. The power operation will inverse the number and then will do a raise to the power of the absolute value if the raise power is negative. The n order root return NR if the number is negative and the order is even. Similar to division, n order root will keep the remainder positive by increasing the absolute value of the result by 1 if necessary. \fprz{n}{r} is similar to \fprn{n}{r}. It use \ipnrz as the value keeper. If the value is using more bits than the size given the number becomes NR.
First NRS of $\mathbb{Q}$ is \ipnrq. It use a fractional system with a numerator and a denominator. The power function treats the negative power the same as \ipnrz. Wen the raise power is of form $\frac{1}{x}$ than the n order root of numerator and denominator is computed. If the form is $\frac{x}{1}$ then both are raised to the power of $X$. In the case where raise power has the form of $\frac{x}{y}$ with $x$ and $y$ different from 1, than first the operation of raising to $x$ is done, and than the result will go though raising to the power of $\frac{1}{y}$. \ipnrq is the first NRS where the Taylor based functions are implemented. The size constrained \fprq{n}{m}{r} use \ipnrq to keep its value. If any of the numerator or denominator goes outside of their given sizes, both are shifted right by 1 until they fit.

\ipnrfixedp keep its value as a \ipnrq. The only requirement for this NRS is that the denominator to be a power of two. \fprfixedp{is}{fs}{r} takes another approach by keeping its value as a \ipnrz. Multiplication is done by multiplying the values and shifting right by fraction size (binary point). The power function is done by separating the raise power in two parts: the integer one and the fractional one. The integer part power is used for accumulating square powers $x, x^2, x^4, ...$, the fractional part is used for accumulating square roots $x, \sqrt{x}, \sqrt{\sqrt{x}}, ...$. The n order root is computed by shifting left the value with $2 \times n$ (g and r) plus $(n-1) \times fraction size$ (to keep the fixed point representation), after the result is shift right by two and than rounded.

\ipnrfloatp keep its exponent value in a \ipnrz and mantissa in a \ipnrfixedp. The power function is done by converting the operands to \ipnrq and than back to \ipnrfloatp after the operation is done.
\floatp{fs} does not have a binary representation, but it is used for implementing other NRSs. It is a super-class NRS. It has a boolean value for the sign, an \ipnrz exponent, a \ipnrn mantissa, some rest bits used for rounding and the fraction size value. It implements all the operation with the scope of having a mantissa in the range $[1,2)$ by making sure that every operations produced at least $fs + 1$ bits of result in mantissa with the most significant one having the value $1$, except for the case when the results is $+0$ or $-0$ and the mantissa is $0$. All the bits remained for the operations are appended in the rest bits list. The power function is similar to \fprfixedp{is}{fs}{r} by separating the integer part and fractional part. This super-class is used further by \fprfloatp{es}{fs}{r} and \fprieee{es}{fs}{r}. \fprfloatp{es}{fs}{r} does the operation using \floatp{fs} and then verifies the results. If the exponent is in the right range than the number is correct. If the exponent is greater than the maximum value it overflows to $\infty$, otherwise if the exponent is lower than the minimum value it underflow to $0$. For binary representation it writes the sign bit, followed by the exponent value in bias form (for $0$ is $0$), and the mantissa bits without the most significant bit. The $\infty$ values are the sign followed only by 1s. For \fprieee{es}{fs}{r} exponent value grater than minimum value or lower than maximum value things goes similar to \fprfloatp{es}{fs}{r}. The $\infty$ values are the sign followed by es of 1s and fs of 0s. If the exponent is greater or equal than maximum exponent value it overflow to $\infty$. If the exponent is lower or equal to minimum exponent value it might be a subnormal number. This is tested by the difference between the subnormal exponent and the exponent value. If it is not a subnormal number it underflow to $0$.

\taperedfloat{size} is similar in computation with \floatp{fs}, but it has dynamic fraction size and additional value which represents size of the NRS. \fprposit{size}{es}{r} and \fprmorris{size}{g}{r} use \taperedfloat{size} for the implementation. \fprposit{size}{es}{r} underflow to the minimum value not $0$ and overflow to the maximum value not $\infty$. \fprmorris{size}{g}{r} underflow to $0$ and overflow to NR. \fprposit{size}{es}{r} is firstly creating the binary representation for the absolute value and than if the sign is negative it subtracts 1 and negate all the bits. The regime bits are the first and than depending on the remaining bits exponent bits followed by mantissa bits without the hidden bit. \fprmorris{size}{g}{r} binary representation starts with the sign than the next g bits represent the minimum size for the exponent absolute value, followed by the exponent sign bit and the exponent bits together with mantissa bits without the hidden bit,

==> nrsold.tex <==
The library implements the NRSs in the Tabel \ref{tab:nrss}. 
\ipnrn influences all the other NRSs. In the current version of the library, \ipnrn takes advantage of \texttt{Scala.BigInt}, improving performance and code readability. \fprn{n}{r} uses \ipnrn to keep the value. Most of the operations use \ipnrn operations in background and the result is converted such that it uses exactly $n$ bits. The results that need more bits are considered Not Representable (NR).

\ipnrz uses \ipnrn to keep the absolute value and a boolean variable for the sign.
For \ipnrz, the euclidean division was chosen because of its mathematical proprieties. The power operation will inverse the number and then will apply power to the absolute value if the power is negative. Similar to division, $n$-order root keeps the remainder positive by increasing the absolute value of the result by one, if necessary. \fprz{n}{r} is similar to \fprn{n}{r}. It uses \ipnrz as the value keeper. If the value is using more bits than the given size, the number becomes NR.

The problem with the fractional system is that it can overflow easy and there are multiple ways to represent the same value. The advantage of the fractional system is that it can represent the entire rational number set $\mathbb{Q}$ in infinite precision. The overflow problem has a partial solution in doing the greater common divisor of the numerator and denominator and dividing both by its value. This solution does not solve the entire problem and adds considerable computation time.
An extension of \fprq{n}{m}{r} proposed to solve the overflow problem is to divide by two (shifting right by one) both the numerator and denominator when one of them is out of the given size. The power function treats the negative power the same as \ipnrz. When the power is of the form $\frac{1}{x}$, the $n$-order root of the numerator and denominator are computed. If the form is $\frac{x}{1}$ then both are raised to the power of $x$. When the power has the form of $\frac{x}{y}$ with $x \neq 1$ and $y \neq 1$, then the operation of raising to $x$ is done first, and then the result is raised to the power of $\frac{1}{y}$. The size-constrained \fprq{n}{m}{r} uses \ipnrq to keep its value.

\textit{fixed point} representation is similar to \textit{2’s complement} integer NRS, but it has an attribute called \textit{binary point}. In a simple way, the value given by the 2’s complement integer NRS is divided by two to the power of the value of the binary point. This system has an overflow problem and a underflow problem. Its range of values is smaller than an integer NRS.
\ipnrfixedp keeps its value as an \ipnrq. The only requirement for this NRS is that the denominator needs to be a power of two. \fprfixedp{is}{fs}{r} takes another approach by keeping its value as a \ipnrz. The power function is done by separating the power into two parts: the integer and the fractional parts. The integer power is used for accumulating square powers ($x, x^2, x^4, ...$), while the fractional power is used for accumulating square roots ($x, \sqrt{x}, \sqrt{\sqrt{x}}, ...$).

In the floating-point system, the number is represented as $(-1)^{sign} \times 2^{exponent}  \times 1.f$. In infinite precision $1.f$ can be seen as a \ipnrfixedp with values inside the $[1,2)$ interval. The first bit represents the sign of the number, the next $es$ (exponent size) bits represent the exponent (usually as a bias integer NRS) and the remaining $fs$ (fraction size) bits represent the fraction bits (usually, there is a hidden bit with the value $1$ which is the most significant bit). The value is given by $(-1)^{sign} \times 2^{exponent}  \times (1+\frac{f}{2^{fs}})$, where $f=\textit{fraction bits value without hidden bit}$. A problem with the floating-point system is that $0$ cannot be represented. A solution is that when all bits except the sign bit are $0s$, the number is $0$. This creates the problem of having $+0$ and $-0$.
Given its infinite precision, \ipnrfloatp does not have the concept of $\infty$.
\floatp{fs} incorporates the concept of $+\infty$ and $-\infty$. The next NRSs are derived from it, with different rules for the range of the exponent, underflow, overflow, rounding, and binary representation. One of these NRSs is \fprfloatp{es}{fs}{r}. \fprfloatp{es}{fs}{r} rules are: (i) in the case of underflow, the value is round to zero when the exponent is smaller than the minimum exponent and the rounding rule does not change this; (ii) in the case of overflow, the value goes to $\infty$ if the exponent value is greater than the maximum exponent; (iii) the exponent is in bias form. To represent $\infty$, all the bits except the sign bit are $1$.

The second floating-point system is the standard called IEEE754~\cite{zuras2008ieee}. This NRS introduced special cases for the smallest and biggest exponent values. When the exponent has the minimum value, the hidden bit is zero and the numbers are called subnormals, except for $+0$ and $-0$. The value of subnormals is given by $(-1)^{sign} \times 2^{\text{-bias}+1} \times (0+\frac{f}{2^{fs}})$, and the process is called gradual underflow. For maximum exponent value, different bit strings for fraction and sign bit can represent \textit{qNaN} (quiet Not A Number - NaN - where the first bit of the fraction is 1), \textit{sNaN} (signal NaN, where the first bit of the fraction is 0, but there is another bit in the fraction different from 0), $+\infty$ (all fraction bits are 0), and $-\infty$ (the same as $+\infty$ only that the sign is negative).

In the library, \floatp{fs} does not have a binary representation, but it is used for implementing other NRSs. It is a super-class NRS. It has a boolean value for the sign, an \ipnrz exponent, a \ipnrn mantissa, some bits used for rounding and the fraction size value. It implements all the operations with the scope of having a mantissa in the range $[1,2)$ by making sure that every operation produces at least $fs + 1$ bits of mantissa with the most significant one having the value $1$, except for the case when the result is $+0$ or $-0$ and the mantissa is $0$. All the additional bits produced by the operation are appended to a rest bits list. The power function is similar to \fprfixedp{is}{fs}{r} by separating the integer and fractional parts of the power. This super-class is used further by \fprfloatp{es}{fs}{r} and \fprieee{es}{fs}{r}. \fprfloatp{es}{fs}{r} and \fprieee{es}{fs}{r} are doing the operations using \floatp{fs} and then verifying the results with their rules for underflow, overflow, and binary representation. Specifically, in the case of \fprieee{es}{fs}{r}, if the exponent is smaller or equal to the minimum exponent value the number might be a subnormal number. This is tested by the difference between the subnormal exponent and the exponent value. If it is not a subnormal number, it underflows to $0$.

Beside issues such as multiple representations for zero, subnormal numbers, and too many bit representations for NaN, IEEE754 might have an oversized or undersized exponent for a given problem. Morris observed this and introduced tapered floating-point \cite{morris1971tapered}, adding an extra field representing the exponent size. This means that the exponent size and the fraction size are dynamically computed. A Morris floating-point system is determined by the bit-width and the size of the exponent denoted by $g$. The first $g$ bits represent the $G$ value which is used to compute the exponent size as $es = G + 1$. The next bit is the exponent sign bit followed by $es$ bits that represent the absolute value of the exponent. The next bit is the fraction sign, and the remaining bits are considered the fraction bits. The hidden bit is always $1$. The final value is computed as $2^{\text{exponent}} \times (-1)^{\textit{fraction sign}} \times (1+\frac{f}{2^{fs}})$, where  $\textit{exponent}=(-1)^{\textit{exponent sign}} \times \textit{exponentBinaryValue}$ (\textit{exponentBinaryValue} is a natural number, not in bias form). Zero is represented by all bits of zero value and error cases (NaN) are represented when all the bits are one. Small numbers have a better precision because more fraction bits are allocated to represent them. In most cases, the dynamic range of Morris NRSs is bigger compared to IEEE754 of the same size, for the obvious reason that more bits can be used for the exponent. On the other hand, these NRSs still have the issue of multiple representations for the same value. Similar to \floatp{fs}, \taperedfloat{size} was created to help with implementing all the operations for tapered floating-point NRSs. In this case, the fraction size is not known so the system uses the bit-width as the exact fraction size. The fraction has a hidden bit with value $1$ and it is in the range $[1,2)$. This NRS does not represent $\infty$. Every NRS derived from it needs to add rules for underflow, overflow, rounding, and binary representation.

In trying to solve the problems of current floating-point systems, Gustafson proposed posit~\cite{gustafson2017beating} (which is another type of \taperedfloat{size}). A posit NRS is determined by its size and exponent size ($es$). The first bit in a posit s-layer representation is the sign bit. The concept for negative numbers is similar with 2's complement: all the bits are negated, and one is added to the value. Next, is the regime field which is dynamic and uses unary arithmetic representation. If the regime starts with a bit $1$, then it is a positive regime and the consecutive $1s$ are counted until a $0$ is found or the end of the representation is reached. The value of the regime is $\text{NoC1} - 1$, where NoC1 is number of consecutive 1s. Otherwise, if the regime starts with a $0$, then it is a negative regime and the consecutive $0s$ are counted until the first bit of $1$ is found or the end of the representation is reached. The regime value in this case is $-1 \times \text{NoC0}$, where NoC0 is number of consecutive 0s. After the regime bits, the next exponent size ($es$) bits represent the exponent value in a base 2 natural number NRS, and the remaining bits are considered fraction bits. The hidden bit is always $1$. The final value of a posit is given by $(-1)^{\textit{sign}} \times 2^{\textit{regime} \times 2^{es} + \textit{exponentBinaryValue}} \times (1+\frac{f}{2^{fs}})$. There are two special cases: for zero, all the bits are $0$, and for $NaR$ (Not a Real - positive infinity and negative infinity), first bit is $1$ and the others are $0$.

Posit solves the problem of a value having multiple representations. This is a strong propriety for an NRS. Like Morris tapered floating-point system, posit has better precision for small number creating a posit ``golden zone'' where all the operations have a better accuracy than other NRSs. \fprposit{n}{es}{r} underflows to the minimum value that is not $0$ and overflows to the maximum value but not $\infty$. \fprmorris{n}{g}{r} underflows to $0$ and overflows to NR. \fprposit{n}{es}{r} is firstly creating the binary representation for the absolute value and then, if the sign is negative it subtracts one and negates all the bits. The regime bits follow the sign bit and then, depending on the remaining bits, we have the exponent bits followed by the fraction bits without the hidden bit. \fprmorris{n}{g}{r} binary representation starts with the sign. The next $g$ bits represent the size for the exponent absolute value, followed by the exponent sign bit, the exponent bits, and the fraction bits without the hidden bit.

\begin{table}
\caption{NRSs implement by the library}\label{tab:nrss}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|p{30em}|}
\hline
\multicolumn{1}{|c|}{\textbf{NRS}} & Description
\\
\hline
\ipnrn & infinite precision without rounding natural number system\\
\hline
\fprn{size}{r} & fixed precision with rounding natural number system, where $size$ is the bit-width and $r$ is the type of rounding\\
\hline
\ipnrz & infinite precision with no rounding sign-magnitude integer number system\\
\hline
\fprz{size}{r} &  fixed precision with rounding integer number system, where $size$ is the bit-width and $r$ is the rounding\\
\hline
\ipnrq & infinite precision with no rounding fractional system\\
\hline
\fprq{n}{m}{r} & fixed precision with rounding fractional system where $n$ is the size of the numerator, $m$ is the size of the denominator, and $r$ is the type of rounding used\\
\hline
\ipnrfixedp & infinite precision with no rounding fixed point system\\
\hline
\fprfixedp{is}{fs}{r} & fixed precision with rounding fixed point system, where $is$ represents the integer size, $fs$ is the binary point value (fraction size), and $r$ is the type of rounding used\\
\hline
\ipnrfloatp & fixed precision with no rounding floating-point number system\\
\hline
\floatp{fs} & floating-point system with infinite precision exponent, no rounding, and with $fs+1$ (fraction size) bits of mantissa (most significant bit always set)\\
\hline
\fprfloatp{es}{fs}{r} & finite precision with rounding floating-point system, where $es$ is the exponent size (exponent in bias form), $fs$ is the fraction size, and $r$ is the type of rounding\\
\hline
\fprieee{es}{fs}{r} & fixed precision with rounding IEEE754 system, where $es$ is the exponent size, $fs$ is the fraction size, and $r$ is the type of rounding\\
\hline
\taperedfloat{size} & tapered floating-point system with infinite precision exponent, no rounding, and with $size$ bits of mantissa with value in $[1,2)$\\
\hline
\fprmorris{size}{g}{r} & fixed precision with rounding Morris tapered floating-point NRS, where $size$ is the bit-width, $g$ is the size of the exponent size, and $r$ is the type of rounding\\
\hline
\fprposit{size}{es}{r} & fixed precision with rounding posit NRS, where $size$ is the bit-width, $es$ is the exponent size, and $r$ is the type of rounding\\
\hline
\end{tabular}
}
\end{table}

==> related.tex <==
https://posithub.org/docs/PDS/PositEffortsSurvey.html
https://arxiv.org/ftp/arxiv/papers/2012/2012.11011.pdf
https://repsy.io/mvn/sdcioc/nrs/ro/upb.nrs
2https://gitlab.com/cerlane/SoftPosit
3https://pypi.org/project/sfpy/
4https://gmplib.org
https://www.nongnu.org/hpalib/

Florent de Dinechin and Bogdan Pasca. Designing custom arithmetic data paths with
%FloPoCo. IEEE Design & Test of Computers, 28(4):18–27, July 2011

Giuseppe Tagliavini, Andrea Marongiu, and Luca Benini. Flexfloat: A software library
for transprecision computing. IEEE Transactions on Computer-Aided Design of Inte-
grated Circuits and Systems, 39(1):145–156, 2018.

Universal: Reliable, Reproducible, and Energy-Efficient Numerics

Small Reals Representations for Deep Learning at the Edge: A Comparison

MULTIPOSITS: Universal Coding of  Rn

https://github.com/stillwater-sc/universal

Granlund, T.: GNU MP. The GNU Multiple Precision Arithmetic Library 2(2) (1996)

 Universal numbers library: design and implementation of a high-performance reproducible number systems library.
 
 https://www.cosic.esat.kuleuven.be/nessie/call/mplibs.html
 
 https://moocaholic.medium.com/fp64-fp32-fp16-bfloat16-tf32-and-other-members-of-the-zoo-a1ca7897d407
 
 https://arxiv.org/pdf/1701.00722.pdf
 
 https://posithub.org/docs/Posits4.pdf
 
 https://marc-b-reynolds.github.io/math/2019/02/06/Posit1.html
 
 What Every Computer Scientist Should Know About Floating-Point Arithmetic David Goldberg
 
 %https://people.eecs.berkeley.edu/~demmel/ma221_Fall20/Dinechin_etal_2019.pdf

%http://www.johngustafson.net/pdfs/BeatingFloatingPoint.pdf
%https://posithub.org/docs/posit_standard-2.pdf

%Next Generation Arithmetic for Edge Computing

%https://dl.acm.org/conference/conga

%https://www.osti.gov/servlets/purl/1866188

% URR: Universal representation of real numbers

% TODO de spus ine valuare ca 0.12109375 12 la suta sunt NAN dintre operatii


